Modelling Privacy Compliance in Cross-border Data Transfers with Bigraphs

Advancements in information technology have led to the sharing of users' data across borders, raising privacy concerns, particularly when destination countries lack adequate protection measures. Regulations like the European General Data Protection Regulation (GDPR) govern international data transfers, imposing significant fines on companies failing to comply. To achieve compliance, we propose a privacy framework based on Milner's Bigraphical Reactive Systems (BRSs), a formalism modelling spatial and non-spatial relationships between entities. BRSs evolve over time via user-specified rewriting rules, defined algebraically and diagrammatically. In this paper, we rely on diagrammatic notations, enabling adoption by end-users and privacy experts without formal modelling backgrounds. The framework comprises predefined privacy reaction rules modelling GDPR requirements for international data transfers, properties expressed in Computation Tree Logic (CTL) to automatically verify these requirements with a model checker and sorting schemes to statically ensure models are well-formed. We demonstrate the framework's applicability by modelling WhatsApp's privacy policies.

==> eptcsdata.tex <==
\providecommand{\firstpage}{17}
\providecommand{\publicationstatus}{J. Endrullis, D. Grzelak, T. Heindel and J. Kosiol (Eds):\\ GCM 2023 and GCM 2024\\
EPTCS 417, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.417.2}{10.4204/EPTCS.417.2}}
\pdfoutput=1

